Hard Thermal Loop -- theory and applications

In this review, we present the key aspects of modern thermal perturbation theory based on the hard thermal loop (HTL) approximation, including its theoretical foundations and applications within quantum electrodynamics (QED) and quantum chromodynamics (QCD) plasmas. To maintain conciseness, we focus on scenarios in thermal equilibrium, examining a variety of physical quantities and settings. Specifically, we explore both bulk thermodynamic properties and real-time observables in high-temperature domains relevant to heavy-ion physics.

==> text/th_field.tex <==
\chapter{Basics of field theory at finite temperature}\label{chap_thft}
%%%
In this chapter we would discuss two formalisms i.e. imaginary time and real time formalism which are used in this thesis. We begin by reviewing the equilibrium statistical thermodynamics. A grand canonical ensemble in equilibrium at finite temperature $T$ is described in terms of the partition function as 
\bea
Z(\beta) &=& \Tr\, \rho(\beta)= \Tr\,{ e^{-\beta (H-\mu N)}},
\eea
where $\beta$ is the inverse of temperature i.e. $\beta=1/T$ and $\mu $ is the chemical potential of the particles is the system. $H$ is the Hamiltonian of the system and $N$ is the number operator. $\rho(\beta)$ is the density matrix. In a canonical ensemble the system is allowed to exchange energy with the heat bath, whereas, in a grand canonical ensemble the system can exchange both energy and particles with the reservoir.
The ensemble average of an observable $\mathcal{O}$ is defined as
\bea
\langle{\mathcal{O}}\rangle_\beta &=&\frac{1}{Z(\beta)} \Tr \, \rho(\beta) \mathcal{O}.
\eea
%%%
 Partition function is important function in thermodynamics and various thermodynamic quantities like pressure $(P)$, entropy density $(S)$, particle number density $(n_i)$ and energy density $(\mathcal{E})$ can be calculated from the following relations:
\bea
P&=& \frac{\partial (T \ln Z)}{\partial V},\\
S&=&  \frac{1}{V}\frac{\partial (T \ln Z)}{\partial T},\\
n_i&=& \frac{1}{V}\frac{\partial (T \ln Z)}{\partial \mu_i},\\
\mathcal{E} &=& -P+T S+ \mu_i N_i,
\eea
where V is the volume of the system. Usually the width of a system is larger than the inverse of the temperature, so that infinite volume limit is taken as a good approximation to describe the thermodynamics.



\section{Imaginary time formalism}
If a Schrodinger operator $\mathcal{O}$ is given, we can define a operator in Heisenberg picture $\mathcal{O}_H(t)$ as 
\bea
\mathcal{O}_H(t)&=&e^{i Ht}\mathcal{O} e^{-iHt}.
\eea

Thermal correlation function of two Heisenberg operators $\mathcal{O}^{1}_H(t)$ and $\mathcal{O}^{2}_H(t')$ can be written as
\bea
\langle\mathcal{O}^{1}_H(t)\mathcal{O}^{2}_H(t')\rangle_\beta &=&Z^{-1}(\beta)\Tr\big[e^{-\beta H}\mathcal{O}^{1}_H(t)\mathcal{O}^{2}_H(t')\big]\nn\\
&=&Z^{-1}(\beta)\Tr\big[e^{-\beta H}\mathcal{O}^{1}_H(t)\,e^{\beta H}e^{-\beta H}\mathcal{O}^{2}_H(t')\big]\nn\\
&=&Z^{-1}(\beta)\Tr\big[\mathcal{O}^{1}_H(t+i\beta)e^{-\beta H}\mathcal{O}^{2}_H(t')\big]\nn\\
&=&Z^{-1}(\beta)\Tr\big[e^{-\beta H}\mathcal{O}^{2}_H(t')\mathcal{O}^{1}_H(t+i\beta)\big]\nn\\
&=&\langle\mathcal{O}^{2}_H(t')\mathcal{O}^{1}_H(t+i\beta)\rangle_\beta .
\label{KMS}
\eea
%%%%%%%%%%%%%%%%%
\begin{figure}[htp]
	\centering
	\includegraphics[width=7.5cm]{Figures/th_field/wick}
	\caption{Wick rotation to imaginary time in complex time plane.}
	\label{wick}
\end{figure}
%%%%%%%%%%%%%%%%%
The cyclic properties of the trace operation is implemented here. The relation of equation~\eqref{KMS} is known as the Kubo-Martin-Schwinger (KMS) relation. This KMS relation leads to the periodicity for bosonic field and the anti-periodicity for fermionic fields in various two point greens functions because of the commutation and anti-commutation relations, respectively. From Eq.~\eqref{KMS} it can be said that the imaginary temperature is connected with the time as $\beta=i t=\tau$. It can be realized by the Wick rotation in complex time plane from Fig.~\ref{wick}. It could be noticed that evolution operator $(e^{-\beta H})$ has the form of time evolution operator $(e^{-i Ht})$ with $\beta=it$. 

The Matsubara (imaginary) time formalism~\cite{10.1143/PTP.14.351} presents a way of evaluating the partition function
using a diagrammatic method.
Now, for a field theory in $(d+1)$ dimensional space-time at finite temperature, the partition function is written as,
\bea
Z(\beta)=\Tr \,e^{-\beta H} =\int \mathcal{D}\phi \exp\bigg[-\int_0^\beta d\tau\int d^d \bold x\ \mathcal{L}(\phi(x))\bigg],
\eea
where $\mathcal{L}$ is the Lagrangian density of the theory. For the bosonic case, the fields obey the periodic boundary condition 
\bea
\phi(0,\bold x)=\phi(\beta, \bold x),
\eea
whereas the fermionic fields obey the anti-periodic boundary conditions
\bea
\phi(0,\bold x)=-\phi(\beta, \bold x).
\eea
%%%%%%%%%%%%

The Feynman rules in finite temperature field theory are same as in zero temperature
except that the imaginary time $\tau$ becomes finite: $0\leq\tau\leq \beta$. Due to the finite range of $\tau$, in the frequency space one has to perform a Fourier series decomposition involving the discrete frequencies. So, the loop frequency integrals are replaced by loop frequency sums:
\bea
\int \frac{d^4 K}{(2\pi)^4} \rightarrow T\sum_{\om_n}\int \frac{d^3k}{(2\pi)^3}
\eea
with the sum over the Matsubara frequencies 
\bea
k_0&=& i\om_n= 2ni \pi T \hspace{2.8cm} \mbox{for bosons},\\
k_0&=&i\om_n= (2n+1)i \pi T +\mu  \hspace{1cm} \mbox{for fermions}.
\eea

\subsection{frequency sums}
\subsubsection{Bosonic case:}
Now we need to perform the the frequency sum. In general the bosonic frequency sum can be written as
\bea
\frac{1}{\beta}\sum_{n=-\infty}^{\infty}f(k_0=i\om_n=2\pi i n T).
\eea
Since hyperbolic cotangent has poles at $n\pi i$ with residue unity, one can insert hyperbolic cotangent with suitable argument as
\bea
\frac{1}{\beta}\sum_{n=-\infty}^{\infty}f(k_0=i\om_n=2\pi i n T) \mbox{Res}\bigg[\frac{\beta}{2}\coth\bigg(\frac{\beta k_0}{2}\bigg)\bigg].
\label{res}
\eea 
Here hyperbolic cotangent corresponds to poles at 
\bea
k_0=\frac{2\pi i n}{\beta}=i\om_n
\eea
with residues $2/\beta$ and as a result $\mbox{Res}\bigg[\frac{\beta}{2}\coth\bigg(\frac{\beta k_0}{2}\bigg)\bigg]$ leads to unity.
From~\eqref{res}, one can write
\bea
\frac{1}{\beta}\sum_{n=-\infty}^{\infty}f(k_0) \mbox{Res}\bigg[\frac{\beta}{2}\coth\bigg(\frac{\beta k_0}{2}\bigg)\bigg]&=&\frac{1}{\beta}\sum_{n=-\infty}^{\infty}\frac{\beta}{2}\mbox{Res}\bigg[f(k_0) \coth\bigg(\frac{\beta k_0}{2}\bigg)\bigg].
\eea
Using the residue theorem the sum over residues can be expressed as an integral over contour $C$ in $\llcorner k_0$ as
\bea
\frac{1}{\beta}\sum_{n=-\infty}^{\infty}\frac{\beta}{2}\mbox{Res}\bigg[f(k_0) \coth\bigg(\frac{\beta k_0}{2}\bigg)\bigg]&=& \frac{1}{2\pi i}\oint\limits_{C}dk_0\frac{1}{2} f(k_0)\coth \bigg(\frac{\beta k_0}{2}\bigg),
\eea
where the contour is shown in Fig.~\ref{contour_boson1}.
%%%%%%%%%%%%%%%%%
\begin{figure}[htp]
	\centering
	\begin{subfigure}[b]{0.41\textwidth}
			\centering
	\includegraphics[width=7.6 cm]{Figures/th_field/contour_boson1}
	\caption{}
	\label{contour_boson1}
\end{subfigure}
\hspace{1.2cm}
	\begin{subfigure}[b]{0.45\textwidth}
	\centering
	\includegraphics[width=6.8cm]{Figures/th_field/contour_boson2}
	\caption{}
	\label{contour_boson2}
\end{subfigure}
	\caption{Contour for bosonic frequency sum.}
\end{figure}
%%%%%%%%%%%%%%%%%
Some important points are noted below:
\begin{itemize}
	\item $\coth(\beta k_0/2)$ is bounded and analytic everywhere except the poles $k_0=i \om_n=2\pi i T$.
	\item The function $f(k_0=i\om_n)$ may have simple poles but no essential singularities or branch cuts.
	\item The function $f(k_0)$ should not have singularities along the imaginary $k_0$ axis.
\end{itemize}
	Now the contour can be deformed as in Fig.~\ref{contour_boson2} dividing the contour $C$ in two half circles $C_1$ and $C_2$ in complex plane $k_0$.
	
	So, the sum integral for the bosonic case can be written as
	\bea
	T\sum_{n=-\infty}^{\infty} f(k_0=i\om_n)&=& \frac{1}{2\pi i}\oint\limits_{C_1\cup C_2}dk_0 f(k_0=i\om_n)\bigg[\frac{1}{2}+\frac{1}{\exp(\beta k_0)-1}\bigg],
	\label{bosonic_sum}
	\eea
	where we used the relation
	\bea
	\coth\bigg(\frac{\beta k_0}{2}\bigg)&=&1+\frac{2}{\exp(\beta k_0)-1}.
	\eea
	It is noted from eq.~\eqref{bosonic_sum}, that the vacuum part $(T=0)$ and medium part $(T\neq 0)$ are separated.

Finally, Eq.~\eqref{bosonic_sum} can be decomposed as 
\bea
T\sum_{n=-\infty}^{\infty} f(k_0=i\om_n)&=& \frac{1}{2\pi i} \int_{-i\infty+\eps}^{i\infty+\eps} dk_0 f(k_0)\bigg[\frac{1}{2}+\frac{1}{\exp(\beta k_0)-1}\bigg]\nn\\
&-& \frac{1}{2\pi i} \int_{i\infty-\eps}^{-i\infty-\eps} dk_0 f(k_0)\bigg[\frac{1}{2}+\frac{1}{\exp(\beta k_0)-1}\bigg].
\eea
Changing variable $k_0\rightarrow -k_0$ in the second integral and using the relation $n_B(-k_0)=-1-n_B(k_0)$, one can write
\bea
T\sum_{n=-\infty}^{\infty} f(k_0=i\om_n)&=& \frac{1}{2\pi i} \int_{-i\infty}^{i\infty} dk_0 \frac{1}{2}[f(k_0)+f(-k_0)]\nn\\
&+& \frac{1}{2\pi i} \int_{-i\infty+\eps}^{i\infty+\eps} dk_0 [f(k_0)+f(-k_0)]n_B(k_0),
\label{contour_boson}
\eea
where $n_B(k_0)=\frac{1}{\exp(\beta k_0)-1}$ is the Bose-Einstein distribution function including the medium effects. We can see that the sum is now converted into a convenient complex integral form. 
\subsubsection{Fermionic case:}
In the similar manner, one can obtain the fermionic frequency sum. The general form of the fermionic frequency sum reads as
\bea
\frac{1}{\beta}\sum_{n=-\infty}^{\infty}f(k_0=i\om_n=(2n+1)\pi i T+\mu).
\eea
As the function $\frac{\beta}{2}\tanh\frac{\beta(p_0-\mu)}{2}$ has poles at $p_0=(2n+1)\pi i T+\mu$ with residue unity, one can put hyperbolic tangent with suitable argument as
\bea
\frac{1}{\beta}\sum_{n=-\infty}^{\infty}f(k_0=i\om_n=(2n+1)\pi i  T+\mu) \mbox{Res}\bigg[\frac{\beta}{2}\tanh\bigg(\frac{\beta (k_0-\mu)}{2}\bigg)\bigg].
\eea
As it is shown for the bosonic case, here we can write the frequency sum as
\bea
&&\frac{1}{\beta}\sum_{n=-\infty}^{\infty}f(k_0=i\om_n=(2n+1)\pi i T+\mu)\nn
\eea
\bea
&=& \frac{1}{2\pi i}\oint\limits_{C}dk_0\frac{1}{2} f(k_0)\tanh \bigg(\beta\,\frac{k_0-\mu}{2}\bigg)\nn\\
&=&\frac{1}{2\pi i}\int_{-i\infty+\mu+\eps}^{i\infty+\mu+\eps}dk_0 f(k_0)\bigg[\frac{1}{2}+\frac{1}{\exp(\beta(k_0-\mu))+1)}\bigg]\nn\\
&-&\frac{1}{2\pi i}\int_{-i\infty+\mu-\eps}^{i\infty+\mu-\eps}dk_0 f(k_0)\bigg[\frac{1}{2}+\frac{1}{\exp(\beta(k_0-\mu))+1)}\bigg].
\eea
After performing the fermionic/bosonic sums, one has to perform the loop momentum integration to calculate several thermodynamic quantities which will be discussed in some next chapters.

%NEED TO CHECK!!!!!!!

\subsection{Saclay Method}
Here, a convenient approach called Saclay-method is discussed to evaluate the frequency sums containing two or more propagators in Feynman loop diagrams. The bosonic propagator $\Delta_B(K)=1/(K^2-m^2)=1/(k_0^2-\bold k^2-m^2)$ in momentum space is written as
\bea
\Delta_B(K)=-\int_0^{\beta} d\tau e^{k_0 \tau} \Delta_B(\tau,E_k),
\eea
where 
\bea
 \Delta_B(\tau,E_k)&=&-T \sum_{k_0=2n\pi i T} e^{-k_0\tau} \Delta_B (K)\nn\\
 &=&\frac{1}{2E_k}\bigg[\{1+n_B(E_k)\}e^{-E_k\tau}+n_B(E_k)e^{E_k\tau}\bigg]\nn\\
 &=&\sum_{s=\pm 1}\frac{s}{2E_k}\{1+n_B(s E_k)\}e^{-sE_k\tau}.
\eea
The above equation can be derived from Eq.~\eqref{contour_boson} using the contour integration.
$E_k=\sqrt{k^2+m^2}$ is the particle energy and
\bea
n_B(E_k)=\frac{1}{e^{\beta E_k}-1}
\eea
denotes the Bose-Einstein distribution.\\
The fermion propagator is represented as
\bea
S(K)=(\slashed K+m)\Delta_F(K).
\eea
The quantity $\Delta_F(K)$ can be written in mixed representation as
\bea
\Delta_F(K)=-\int_0^{\beta} d\tau e^{k_0 \tau} \Delta_F(\tau,E_k),
\eea
where
\bea
\Delta_F(\tau,E_k)&=&-T \sum_{k_0=(2n+1)\pi i T} e^{-k_0\tau} \Delta_F (K)\nn\\
&=&\sum_{s=\pm 1}\frac{s}{2E_k}\{1-n_F(s E_k)\}e^{-sE_k\tau}.
\label{delF}
\eea
$n_F(E_k)=\frac{1}{e^{\beta E_k}+1}$ is the Fermi-Dirac distribution. 
\subsubsection{Evolution of frequency sums:}
We discuss the fermion-antifermion case. This kind of situation appears in gauge-boson self-energy calculation where the external line is a bosonic line.
\subsubsection{1. Evolution of $T\sum_{k_0}\Delta_F(K)\Delta_F(Q)$:}
\bea
&&T\sum_{k_0=(2n+1)i\pi T} \Delta_F(K)\Delta_F(Q=P-K)\nn\\
&=& T\sum_{k_0}\int_0^\beta d\tau \int_0^\beta d\tau' e^{k_0\tau}\Delta_F(\tau,E_k)e^{q_0\tau'}\Delta_F(\tau',E_q)\nn\\
&=&\int d\tau \int d\tau' e^{p_0\tau'}T\sum_{k_0}e^{k_0(\tau-\tau')}\Delta_F(\tau,E_k)\Delta_F(\tau',E_q)\nn\\
&=&\int d\tau \int d\tau' e^{p_0\tau'}\delta(\tau-\tau')\Delta_F(\tau,E_k)\Delta_F(\tau',E_q)\nn\\
&=&\int d\tau e^{p_0\tau}\Delta_F(\tau,E_k)\Delta_F(\tau,E_q)\nn\\
&=&\sum_{s_1,s_2}\frac{s_1 s_2}{4E_k E_q}\int d\tau\,  e^{p_0\tau}[1-n_F(s_1 E_k)][1-n_F(s_2 E_q)]e^{-s_1E_k-s_2E_q}\tau\nn\\
&=&-\sum_{s_1,s_2}\frac{s_1 s_2}{4E_k E_q}\frac{1-n_F(s_1E_k)-n_F(s_2E_q)}{p_0-s_1E_k-s_2 E_q}.
\eea
\subsubsection{2. Evolution of $T\sum_{k_0}k_0\Delta_F(K)\Delta_F(Q)$:}
\bea
&&T\sum_{k_0=(2n+1)i\pi T}k_0 \Delta_F(K)\Delta_F(Q=P-K)\nn\\
&=& T\sum_{k_0}\int_0^\beta d\tau \int_0^\beta d\tau' \frac{\partial}{\partial \tau}(e^{k_0\tau})\Delta_F(\tau,E_k)e^{q_0\tau'}\Delta_F(\tau',E_q)\nn\\
&=& T\sum_{k_0}\int \frac{\partial}{\partial \tau}(e^{k_0\tau})\Delta_F(\tau,E_k)d\tau \int d\tau' e^{q_0\tau'}\Delta_F(\tau',E_q).
\label{evo_2}
\eea
We Use integration by parts to simplify the last line,
\bea
\int_0^\beta \frac{\partial}{\partial \tau}(e^{k_0\tau})\Delta_F(\tau,E_k)d\tau&=&\Delta_F(\tau,E_k)e^{k_0\tau}\bigg|_0^\beta-\int_0^\beta e^{k_0\tau}\frac{\partial}{\partial \tau}\Delta_F(\tau,E_k)d\tau\nn\\
&=&-[\Delta_F(\beta,E_k)+\Delta_F(0,E_k)]-\int_0^\beta e^{k_0\tau}\frac{\partial}{\partial \tau}\Delta_F(\tau,E_k)d\tau\nn\\
&=&-\int_0^\beta e^{k_0\tau}\frac{\partial}{\partial \tau}\Delta_F(\tau,E_k)d\tau.
\label{bypartsdelF}
\eea
We have used $e^{k_0\beta}=-1$. By using Eq.~\eqref{delF}, It is also easy to show that the terms in the third bracket of the second line of Eq.~\eqref{bypartsdelF} give zero.
Putting Eq.~\eqref{bypartsdelF} in Eq.~\eqref{evo_2} we get,
\bea
&&T\sum_{k_0=(2n+1)i\pi T}k_0 \Delta_F(K)\Delta_F(Q)\nn\\
&=& T\sum_{k_0}\int_0^\beta d\tau \int_0^\beta d\tau' e^{k_0\tau}\frac{\partial}{\partial \tau}\Delta_F(\tau,E_k)e^{q_0\tau'}\Delta_F(\tau',E_q)\nn\\
&=&\int d\tau \int d\tau' e^{p_0\tau'}T\sum_{k_0}e^{k_0(\tau-\tau')}\frac{\partial}{\partial \tau}\Delta_F(\tau,E_k)\Delta_F(\tau',E_q)\nn\\
&=&\int d\tau \int d\tau' e^{p_0\tau'}\delta(\tau-\tau')\frac{\partial}{\partial \tau}\Delta_F(\tau,E_k)\Delta_F(\tau',E_q)\nn\\
&=&\int d\tau e^{p_0\tau}\frac{\partial}{\partial \tau}\Delta_F(\tau,E_k)\Delta_F(\tau,E_q)\nn\\
&=-&\sum_{s_1,s_2}\frac{ s_2}{4E_q}\int d\tau\,  e^{p_0\tau}[1-n_F(s_1 E_k)][1-n_F(s_2 E_q)]e^{-s_1E_k-s_2E_q}\tau\nn\\
&=&\sum_{s_1,s_2}\frac{ s_2}{4 E_q}\frac{1-n_F(s_1E_k)-n_F(s_2E_q)}{p_0-s_1E_k-s_2 E_q}.
\eea
We have used here $e^{p_0\beta}=1$ as the external line is a bosonic line i.e. $p_0=2\pi i n T $. 



\section{Real time formalism}
Imaginary time formalism is applied to study the static and equilibrium properties of a system. The time dependence appears non-trivially through the analytical continuation. This formalism cannot describe the out of equilibrium systems. On the other hand, real time formalism is appropriate framework to handle the out of equilibrium systems and also to study the dynamical situations such as phase transition or evolution of the universe. 

The real time formalism was originally proposed by Schwinger and Keldysh~\cite{Schwinger:1960qe,Keldysh:1964ud}. Here we briefly discuss the real time method~\cite{Das:1997gg, mallik_sarkar_2016, Bellac:2011kqa}. For better understanding we start with quantum mechanics. At finite temperature $\beta^{-1}=T$, the one important quantity is the partition function
\bea
\Tr e^{-\beta H}=\int_{-\infty}^{\infty} dq \braket{q,t|e^{-\beta H}|q,t}.
\label{partition_func}
\eea
This is the analogous to the transition amplitude for a system from $q$ at time $t$ to $q'$ at time $t'$ in vacuum theory
\bea
 \braket{q',t'|q,t}=\braket{q',t'|e^{-i H(t'-t)}|q,t},
\eea
where $H$ is the Hamiltonian of the system. The operator $e^{-iH(t'-t)}$ corresponds that the system evolves from time $t$ to $t'$. Similarly, drawing the analogy with the vacuum case, one can think that the operator $e^{-\beta H}=e^{-iH(\tau-i\beta-\tau)}$ evolves the system from time $\tau$ to $\tau-i\beta$ in the complex time path $C$.

Thermal scalar field propagator is defined as 
\bea
D(x,x')&=&i\langle T\phi(x)\phi(x')\rangle\nn\\
&=&\theta(\tau-\tau')i \langle \phi(x)\phi(x')\rangle+\theta(\tau'-\tau)i \langle \phi(x')\phi(x)\rangle,\nn\\
&=&\theta(\tau-\tau')D_+(x,x')+\theta(\tau'-\tau)D_-(x,x').
\eea
$\tau$ and $\tau'$ are the points on the contour. $\theta(\tau-\tau')$ is the contour-odered theta function. $D_+(\bold x, \bold x'; \tau,\tau')$ is defined in domain $-\beta\leq \text{Im}(\tau-\tau')\leq 0$ whereas, $D_-(\bold x, \bold x'; \tau,\tau')$ is defined in domain $\beta\geq \text{Im}(\tau-\tau')\geq 0$. The thermal propagator satisfy the equation
\bea
(\square^2+m^2)D(x,x')=\delta^4(x-x'),
\eea
with boundary condition
\bea
D_-(\bold x,\bold x';\tau,\tau')=D_+(\bold x,\bold x';\tau-i\beta,\tau')
\eea
known as KMS relation (shown in Eq.~\eqref{KMS}).
Going to the spacial Fourier transform space and solving the differential equation one can easily get
\bea
D(\bold k;\tau-\tau')=\frac{i}{2\om}\bigg\{\big[\theta(\tau-\tau')+n_B\big]e^{-i\om(\tau-\tau')}+\big[\theta(\tau'-\tau)+n_B\big]e^{i\om(\tau-\tau')}\bigg\},
\eea
where $n_B(\om)=\frac{1}{e^{\beta \om}-1}$ is the single particle thermal distribution function with $\om^2=\bold k^2+m^2$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htp]
	\centering
	\includegraphics[width=14cm]{Figures/th_field/time1}
	\caption{The contour for the real time formalism.}
	\label{contour_realtime}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Now we need to specify the contour and the suitable choice is shown in Fig.~\ref{contour_realtime}. The path traverses from $-\bar t$ to $+\bar t$ in real axis, then it continues in vertical path from $\bar t$ to $\bar t-i\beta/2$. Then it runs from parallel to real axis upto $-\bar t-i\beta/2$ and finally takes the vertical path upto $-\bar t-i\beta$.

$D(\bold k, \tau_h,\tau_v)\rightarrow 0$ by Riemann-Lebesgue lemma where $\tau_v$ and $\tau_h$ are points point on vertical and horizontal lines respectively. Both points on vertical lines are not considered as we are interested only in propagator having points on real axis. So, we are left with two lines parallel to real axes and the propagator can be written in form of $2\times 2$ matrix. The propagator is given in $ij$-th element as 
\bea
D(\bold k;\tau_i-\tau'_j)=\frac{i}{2\om}\bigg\{\big[\theta(\tau_i-\tau'_j)+n_B\big]e^{-i\om(\tau_i-\tau'_j)}+\big[\theta(\tau'_j-\tau_i)+n_B\big]e^{i\om(\tau_i-\tau'_j)}\bigg\}.
\eea
Now we can write down the contour ordering in terms of the usual time $(t)$ ordering.
When $\tau $ and $\tau'$ are on line $1$ (real axis from $-\bar t$ to $\bar t$), $\theta(\tau_1-\tau_1')=\theta(t-t')$. If $\tau $ and $\tau'$ are on line $2$ (real axis from $\bar t-i\beta/2$ to $-\bar t-i\beta/2$), it is written as $\theta(\tau_2-\tau_2')=\theta(t'-t)$. When the points are on different lines, we note that $\theta(\tau_1-\tau_2')=0$ and $\theta(\tau_2-\tau_1')=1$.

Now the components of propagator in the momentum space are written by taking temporal Fourier transform as
\bea
D_{ij}(\bold k,k_0)=\int_{-\infty}^{\infty} e^{ik_0 (t-t')} D(\bold k;\tau_i,\tau_j')dt.
\eea
Performing the integration, they can take the forms
\bea
D_{11}&=&\Delta_F(k)+2i\pi n_B(\om)\delta(k^2-m^2),\\
D_{12}&=&2i\pi \sqrt{n_B(\om)(1+n_B(\om))}\delta(k^2-m^2),
\eea
whereas the other components are written as
\bea
D_{21}&=&D_{12},\nn\\
D_{22}&=&-D_{11}^*.
\eea
Finally, we can write the momentum space scalar propagator in terms of matrix as
\bea
D(k_0,\bold k)=
\begin{bmatrix}
	\Delta_F(k)+2i\pi n_B\delta(k^2-m^2) & 2i\pi \sqrt{n_B(1+n_B)}\delta(k^2-m^2)\\
	2i\pi \sqrt{n_B(1+n_B)}\delta(k^2-m^2) & 	-\Delta_F(k)^*+2i\pi n_B\delta(k^2-m^2) 
\end{bmatrix},
\eea
where $	\Delta_F(k)$ is the free scalar propagator. We use real time formalism to calculate gluon self-energy in chapter~\ref{chapter_1}.








